Security Update Labels: Establishing Economic Incentives for Security Patching of IoT Consumer Products

With the expansion of the Internet of Things (IoT), the number of security incidents due to insecure and misconfigured IoT devices is increasing. Especially on the consumer market, manufacturers focus on new features and early releases at the expense of a comprehensive security strategy. Hence, experts have started calling for regulation of the IoT consumer market, while policymakers are seeking for suitable regulatory approaches. We investigate how manufacturers can be incentivized to increase sustainable security efforts for IoT products. We propose mandatory security update labels that inform consumers during buying decisions about the willingness of the manufacturer to provide security updates in the future. Mandatory means that the labels explicitly state when security updates are not guaranteed. We conducted a user study with more than 1,400 participants to assess the importance of security update labels for the consumer choice by means of a conjoint analysis. The results show that the availability of security updates (until which date the updates are guaranteed) accounts for 8% to 35% impact on overall consumers' choice, depending on the perceived security risk of the product category. For products with a high perceived security risk, this availability is twice as important as other high-ranked product attributes. Moreover, provisioning time for security updates (how quickly the product will be patched after a vulnerability is discovered) additionally accounts for 7% to 25% impact on consumers' choices. The proposed labels are intuitively understood by consumers, do not require product assessments by third parties before release, and have a potential to incentivize manufacturers to provide sustainable security support.

==> sections/tables/table-attribute-descriptions.tex <==
\begin{table}
  \centering
  \captionof{table}{Description of attributes. \philipp{Need to be fixed after focus group interviews.}}
  \label{tab:attributes:description}
  \begin{tabular}{@{}p{2cm} p{6cm}}
    \toprule
    \bf Attribute & \bf Description \\
    \midrule
	Security Lifetime & Overall time period that the manufacturer guarantees to deliver software updates. \\
	\midrule
	Time-to-Patch & Allowed time span until software update is available after security bug was disclosed. \\
	\midrule
	... & ...\\
    \bottomrule
  \end{tabular}
\end{table}

==> sections/tables/table-further-utilities.tex <==
\begin{table}
  \centering
  \captionof{table}{Average utilities (zero-sum) of remaining product attributes. }
  \label{tab:utilities-appendix}
  \setlength{\tabcolsep}{3pt}
  \begin{tabular}{@{}l l r r@{}}
  \toprule
  \bf \multirow{2}{*}{Attribute} & \bf \multirow{2}{*}{Level} & \multicolumn{1}{R{1.6cm}}{\bf Smart Home Camera} & \multicolumn{1}{R{1.9cm}@{}}{\bf Smart Weather Station}\\
   \midrule
    	\multirow{2}{*}{Resolution}
    	& HD & -39.36 &   \\
    	& Full-HD & 39.36 &   \\
   \midrule
    	\multirow{3}{*}{Field of view}
    	& 110\textdegree & -28.27 & -  \\
    	& 130\textdegree & 3.60 & -  \\
    	& 150\textdegree & 24.67 & -  \\
   \midrule
    	\multirow{3}{*}{Frame rate}
    	& 25fps & -32.24 & -  \\
    	& 30fps & -1.56 & - \\
    	& 50fps & 33.80 & -   \\
   \midrule
    	\multirow{2}{*}{Zoom function}
    	& yes & 28.05 & -  \\
    	& no & -28.05 & -  \\
   \midrule
    	\multirow{3}{*}{Battery lifetime}
    	& 1 year & - & -34.43  \\
    	& 2 years & - & 7.37  \\
    	& 3 years & - & 27.06  \\
   \midrule
    	\multirow{3}{*}{Precision}
    	& $\pm$0.2\textdegree{}C & - & 17.10  \\
    	& $\pm$0.3\textdegree{}C & - & 6.19  \\
    	& $\pm$0.5\textdegree{}C & - & -23.29  \\
   \midrule
    	\multirow{2}{*}{Rain/wind sensor}
    	& yes & - & 54.30   \\
    	& no & - & -54.30  \\
   \midrule
    	\multirow{2}{*}{Expandability}
    	& yes & - &  43.66 \\
    	& no & - & -43.66  \\
%   \midrule
%    	\multirow{1}{*}{None}
%    	&  & -94.46  &  -36.37 \\
    \bottomrule
  \end{tabular}
%  \begin{tablenotes}
%      \footnotesize
%      \item The average utilities of the further attributes are shown in \Cref{tab:utilities}.
%  \end{tablenotes}
\end{table}


==> sections/tables/table-segmentation.tex <==
\begin{table*}
  \centering
  \captionof{table}{Consumer segmentation via latent-class analysis.}
  \label{tab:segmentation}
  \setlength{\tabcolsep}{4pt}
  \begin{tabular}{l l r r l r r l}
    \toprule
    \multirow{6}{*}{\bf } & &  \multicolumn{3}{c}{\bf Smart Home Camera}  &  \multicolumn{3}{c}{\bf Smart Weather Station} \\
    \cmidrule(l){3-5}
    \cmidrule(l){6-8}
    & \multicolumn{1}{r}{\it} & \it Group 1 & \it Group 2 &  & \it Group 1 & \it Group 2 & \\ 
    \cmidrule{1-2}
    \cmidrule(l){3-4}
    \cmidrule(l){6-7}
     & \multicolumn{1}{r}{n} & 488 & 243 & \it Group 1 versus Group 2 & 542 & 193 & \it Group 1 versus Group 2  \\ 
    \cmidrule{1-2}
    \cmidrule(l){3-4}
    \cmidrule(l){5-5}
    \cmidrule(l){6-7}
    \cmidrule(l){8-8}
	\multirow{2}{*}{Gender} 
	& female 			& 42.6\% & 44.9\%  & \multirow{2}{*}{${\chi}^2(1) = 0.42, \phi = 0.090$} & 44.3\%  & 43.0\% & \multirow{2}{*}{${\chi}^2(1) = 0.12, \phi = 0.090$}\\ 
	& male  				& 55.9\%  & 53.1\% &  & 55.0\%  & 54.4\% &  \\ 
    \cmidrule{1-2}
    \cmidrule(l){3-4}
    \cmidrule(l){5-5}
    \cmidrule(l){6-7}
    \cmidrule(l){8-8}
	\multirow{1}{*}{Age} 
	& $\mu$  [years]			& 33.0 & 33.9 & $t(729) = -1.10, d = -0.09$ & 33.6 & 36.7 &  $t(733) = -3.30\textsuperscript{**}, d = -0.28$  \\ 
    \cmidrule{1-2}
    \cmidrule(l){3-4}
    \cmidrule(l){5-5}
    \cmidrule(l){6-7}
    \cmidrule(l){8-8}
 	\multirow{3}{1.7cm}{Vocational qualification} 
	& none 				 & 9.2\%   & 11.9\%  & & 12.0\%   & 8.8\% &  \\ 
	& vocational-oriented	 & 38.7\%  & 42.8\% & ${\chi}^2(2) = 3.35, \phi =0.068$ & 39.5\%  & 38.9\% &  ${\chi}^2(2) = 1.72, \phi = 0.048$ \\ 
	& academic			 & 52.0\%  & 45.3\% & & 48.5\%  & 52.3\% &  \\ 
% https://www.socscistatistics.com/tests/chisquare2
% P1: The chi-square statistic is 3.3477. The p-value is .187524. The result is not significant at p < .05.
% P2: The chi-square statistic is 1.7242. The p-value is .422266. The result is not significant at p < .05.
    \cmidrule{1-2}
    \cmidrule(l){3-4}
    \cmidrule(l){5-5}
    \cmidrule(l){6-7}
    \cmidrule(l){8-8}
 	\multirow{1}{2.7cm}{Monthly net income} 
	& $\mu$	 [\euro{}]			& 1667   & 1681  &   $t(599) = -0.14, d = -0.01$ & 1365  & 1622 &  $t(529) = -2.45\textsuperscript{*}, d = 0.26$ \\ 
    \cmidrule{1-2}
    \cmidrule(l){3-5}
    \cmidrule(l){6-8}
 	\multirow{2}{1.7cm}{Professional IT background} 
	& yes 				& 18.5\%  & 17.7\%  & \multirow{2}{*}{${\chi}^2(1) = 0.06, \phi = 0.010$} & 17.6\%  & 15.2\% & \multirow{2}{*}{${\chi}^2(1) = 0.57, \phi = 0.028$} \\ 
	& no  				& 81.5\%  & 82.3\%  & & 82.4\%  & 84.8\% &  \\ 
    \cmidrule{1-2}
    \cmidrule(l){3-4}
    \cmidrule(l){5-5}
    \cmidrule(l){6-7}
    \cmidrule(l){8-8}
	\multicolumn{2}{l}{Privacy concerns} 	& 4.48 & 4.59 &  $t(729) = -0.98, d = -0.08$ & 4.37 & 4.56 &  $t(733) = -1.58, d = -0.13$ \\ 
	\multicolumn{2}{l}{Security behavior intention} 	 & 3.59 & 3.56 &  $t(729) = 0.59, d = 0.05$ & 3.55 & 3.69 &  $t(733) = -2.75\textsuperscript{**}, d = -0.23$ \\ 
    \cmidrule{1-2}
    \cmidrule(l){3-4}
    \cmidrule(l){5-5}
    \cmidrule(l){6-7}
    \cmidrule(l){8-8}
     	 \multicolumn{2}{l}{Perceived security risk} 
				& 5.44 & 5.61 &  $t(729) = -2.13\textsuperscript{*}, d = -0.17$ & 3.56 & 3.90 &  $t(733) = -2.78\textsuperscript{**}, d = -0.23$\\ 
    \bottomrule
  \end{tabular}
   \begin{tablenotes}
      \footnotesize
      \item Notation: Statistically significant with \textsuperscript{*}$p<0.05$, \textsuperscript{**}$p<0.01$
  \end{tablenotes}
\end{table*}


\begin{table}
  \centering
  \captionof{table}{Product attribute importance of consumer groups. }
  \label{tab:segmentation2}
  \setlength{\tabcolsep}{6.3pt}
  \begin{tabular}{c l r l r}
    \toprule
    & \multicolumn{4}{c}{\bf Smart Home Camera}  \\
    %\cmidrule(){1-1}
    \cmidrule(l){2-5}
    \it Rank & \multicolumn{2}{c}{\it Group 1 (n = 488)} & \multicolumn{2}{c}{\it Group 2 (n = 243)}  \\ 
    \cmidrule(){1-1}
    \cmidrule(l){2-3}
    \cmidrule(l){4-5}
	1. & Availability\textsuperscript{1}  			& 31.42\%  & Availability\textsuperscript{1}  & 25.26\%  \\ 
	2. & Resolution  			& 16.47\% & Provisioning time\textsuperscript{2}  & 19.03\%   \\ 
	3. & Price 				& 11.82\%  & Price & 16.66\%   \\ 
	4. & Frame rate  			& 10.68\%  & Field of view & 11.64\%   \\  
	5. & Zoom function  		& 10.48\%   & Frame rate & 9.26\%   \\ 
	6. & Provisioning time\textsuperscript{2} 	& 10.22\%  & Resolution & 9.17\%  \\ 
	7. & Field of view  		& 8.91\%  & Zoom function & 8.98\%   \\
    \midrule
    & \multicolumn{4}{c}{\bf Smart Weather Station}  \\
    %\cmidrule(){1-1}
    \cmidrule(l){2-5}
    \it Rank & \multicolumn{2}{c}{\it Group 1 (n = 542)} & \multicolumn{2}{c}{\it Group 2 (n = 193)}  \\ 
    \cmidrule(){1-1}
    \cmidrule(l){2-3}
    \cmidrule(l){4-5}
	1. & Price 				& 19.52\%  & Availability\textsuperscript{1} 		& 23.91\%   \\
	2. & Availability\textsuperscript{1} 		& 19.32\%  & Rain/wind sensor  	& 22.12\%   \\  
	3. & Rain/wind sensor  	& 15.06\%  & Provisioning time\textsuperscript{2}  	& 19.98\%   \\
	4. & Provisioning time\textsuperscript{2}  	& 14.45\%  & Expandability  		& 15.84\%   \\ 
	5. & Expandability  		& 12.92\%  & Price 				& 8.46\%   \\ 
	6. & Battery Lifetime  	& 11.37\%  & Battery Lifetime  	& 5.38\%   \\ 
	7. & Precision		 	& 7.36\%    & Precision		 	& 4.31\%   \\ 
    \bottomrule
  \end{tabular}
   \begin{tablenotes}
      \footnotesize
      \item \textsuperscript{1}Availability of security updates, \textsuperscript{2}Provisioning time for security updates
  \end{tablenotes}
\end{table}




% Eventuell später: https://tex.stackexchange.com/questions/211898/putting-several-footnotes-below-the-table?rq=1
